Simultaneous Multi Layer Access: A High Bandwidth and Low Cost 3D-Stacked Memory Interface

Limited memory bandwidth is a critical bottleneck in modern systems. 3D-stacked DRAM enables higher bandwidth by leveraging wider Through-Silicon-Via (TSV) channels, but today's systems cannot fully exploit them due to the limited internal bandwidth of DRAM. DRAM reads a whole row simultaneously from the cell array to a row buffer, but can transfer only a fraction of the data from the row buffer to peripheral IO circuit, through a limited and expensive set of wires referred to as global bitlines. In presence of wider memory channels, the major bottleneck becomes the limited data transfer capacity through these global bitlines. Our goal in this work is to enable higher bandwidth in 3D-stacked DRAM without the increased cost of adding more global bitlines. We instead exploit otherwise-idle resources, such as global bitlines, already existing within the multiple DRAM layers by accessing the layers simultaneously. Our architecture, Simultaneous Multi Layer Access (SMLA), provides higher bandwidth by aggregating the internal bandwidth of multiple layers and transferring the available data at a higher IO frequency. To implement SMLA, simultaneous data transfer from multiple layers through the same IO TSVs requires coordination between layers to avoid channel conflict. We first study coordination by static partitioning, which we call Dedicated-IO, that assigns groups of TSVs to each layer. We then provide a simple, yet sophisticated mechanism, called Cascaded-IO, which enables simultaneous access to each layer by time-multiplexing the IOs. By operating at a frequency proportional to the number of layers, SMLA provides a higher bandwidth (4X for a four-layer stacked DRAM). Our evaluations show that SMLA provides significant performance improvement and energy reduction (55%/18% on average for multi-programmed workloads, respectively) over a baseline 3D-stacked DRAM with very low area overhead.

==> log <==
This is pdfTeX, Version 3.1415926-2.5-1.40.14 (TeX Live 2013/Debian) (format=pdflatex 2014.11.5)  9 JUN 2015 23:09
entering extended mode
 restricted \write18 enabled.
 %&-line parsing enabled.
**paper
(./paper.tex
LaTeX2e <2011/06/27>
Babel <3.9h> and hyphenation patterns for 78 languages loaded.
(/usr/share/texlive/texmf-dist/tex/latex/base/article.cls
Document Class: article 2007/10/19 v1.4h Standard LaTeX document class
(/usr/share/texlive/texmf-dist/tex/latex/base/size10.clo
File: size10.clo 2007/10/19 v1.4h Standard LaTeX file (size option)
)
\c@part=\count79
\c@section=\count80
\c@subsection=\count81
\c@subsubsection=\count82
\c@paragraph=\count83
\c@subparagraph=\count84
\c@figure=\count85
\c@table=\count86
\abovecaptionskip=\skip41
\belowcaptionskip=\skip42
\bibindent=\dimen102
)
(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphicx.sty
Package: graphicx 1999/02/16 v1.0f Enhanced LaTeX Graphics (DPC,SPQR)

(/usr/share/texlive/texmf-dist/tex/latex/graphics/keyval.sty
Package: keyval 1999/03/16 v1.13 key=value parser (DPC)
\KV@toks@=\toks14
)
(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphics.sty
Package: graphics 2009/02/05 v1.0o Standard LaTeX Graphics (DPC,SPQR)

(/usr/share/texlive/texmf-dist/tex/latex/graphics/trig.sty
Package: trig 1999/03/16 v1.09 sin cos tan (DPC)
)
(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/graphics.cfg
File: graphics.cfg 2010/04/23 v1.9 graphics configuration of TeX Live
)
Package graphics Info: Driver file: pdftex.def on input line 91.

(/usr/share/texlive/texmf-dist/tex/latex/pdftex-def/pdftex.def
File: pdftex.def 2011/05/27 v0.06d Graphics/color for pdfTeX

(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/infwarerr.sty
Package: infwarerr 2010/04/08 v1.3 Providing info/warning/error messages (HO)
)
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/ltxcmds.sty
Package: ltxcmds 2011/11/09 v1.22 LaTeX kernel commands for general use (HO)
)
\Gread@gobject=\count87
))
\Gin@req@height=\dimen103
\Gin@req@width=\dimen104
)
(/usr/share/texlive/texmf-dist/tex/latex/url/url.sty
\Urlmuskip=\muskip10
Package: url 2013/09/16  ver 3.4  Verb mode for urls, etc.
)
(/usr/share/texlive/texmf-dist/tex/latex/pslatex/pslatex.sty
Package: pslatex 1996/07/24 v1.2 pslatex emulation (DPC)
LaTeX Font Info:    Redeclaring symbol font `operators' on input line 65.
LaTeX Font Info:    Overwriting symbol font `operators' in version `normal'
(Font)                  OT1/cmr/m/n --> OT1/ptmcm/m/n on input line 65.
LaTeX Font Info:    Overwriting symbol font `operators' in version `bold'
(Font)                  OT1/cmr/bx/n --> OT1/ptmcm/m/n on input line 65.
LaTeX Font Info:    Redeclaring symbol font `letters' on input line 66.
LaTeX Font Info:    Overwriting symbol font `letters' in version `normal'
(Font)                  OML/cmm/m/it --> OML/ptmcm/m/it on input line 66.
LaTeX Font Info:    Overwriting symbol font `letters' in version `bold'
(Font)                  OML/cmm/b/it --> OML/ptmcm/m/it on input line 66.
LaTeX Font Info:    Redeclaring symbol font `symbols' on input line 67.
LaTeX Font Info:    Overwriting symbol font `symbols' in version `normal'
(Font)                  OMS/cmsy/m/n --> OMS/pzccm/m/n on input line 67.
LaTeX Font Info:    Overwriting symbol font `symbols' in version `bold'
(Font)                  OMS/cmsy/b/n --> OMS/pzccm/m/n on input line 67.
LaTeX Font Info:    Redeclaring symbol font `largesymbols' on input line 68.
LaTeX Font Info:    Overwriting symbol font `largesymbols' in version `normal'
(Font)                  OMX/cmex/m/n --> OMX/psycm/m/n on input line 68.
LaTeX Font Info:    Overwriting symbol font `largesymbols' in version `bold'
(Font)                  OMX/cmex/m/n --> OMX/psycm/m/n on input line 68.
\symbold=\mathgroup4
\symitalic=\mathgroup5
LaTeX Font Info:    Redeclaring math alphabet \mathbf on input line 74.
LaTeX Font Info:    Overwriting math alphabet `\mathbf' in version `normal'
(Font)                  OT1/cmr/bx/n --> OT1/ptm/bx/n on input line 74.
LaTeX Font Info:    Overwriting math alphabet `\mathbf' in version `bold'
(Font)                  OT1/cmr/bx/n --> OT1/ptm/bx/n on input line 74.
LaTeX Font Info:    Redeclaring math alphabet \mathit on input line 75.
LaTeX Font Info:    Overwriting math alphabet `\mathit' in version `normal'
(Font)                  OT1/cmr/m/it --> OT1/ptm/m/it on input line 75.
LaTeX Font Info:    Overwriting math alphabet `\mathit' in version `bold'
(Font)                  OT1/cmr/bx/it --> OT1/ptm/m/it on input line 75.
)
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsmath.sty
Package: amsmath 2013/01/14 v2.14 AMS math features
\@mathmargin=\skip43

For additional information on amsmath, use the `?' option.
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amstext.sty
Package: amstext 2000/06/29 v2.01

(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsgen.sty
File: amsgen.sty 1999/11/30 v2.0
\@emptytoks=\toks15
\ex@=\dimen105
))
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsbsy.sty
Package: amsbsy 1999/11/29 v1.2d
\pmbraise@=\dimen106
)
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsopn.sty
Package: amsopn 1999/12/14 v2.01 operator names
)
\inf@bad=\count88
LaTeX Info: Redefining \frac on input line 210.
\uproot@=\count89
\leftroot@=\count90
LaTeX Info: Redefining \overline on input line 306.
\classnum@=\count91
\DOTSCASE@=\count92
LaTeX Info: Redefining \ldots on input line 378.
LaTeX Info: Redefining \dots on input line 381.
LaTeX Info: Redefining \cdots on input line 466.
\Mathstrutbox@=\box26
\strutbox@=\box27
\big@size=\dimen107
LaTeX Font Info:    Redeclaring font encoding OML on input line 566.
LaTeX Font Info:    Redeclaring font encoding OMS on input line 567.
\macc@depth=\count93
\c@MaxMatrixCols=\count94
\dotsspace@=\muskip11
\c@parentequation=\count95
\dspbrk@lvl=\count96
\tag@help=\toks16
\row@=\count97
\column@=\count98
\maxfields@=\count99
\andhelp@=\toks17
\eqnshift@=\dimen108
\alignsep@=\dimen109
\tagshift@=\dimen110
\tagwidth@=\dimen111
\totwidth@=\dimen112
\lineht@=\dimen113
\@envbody=\toks18
\multlinegap=\skip44
\multlinetaggap=\skip45
\mathdisplay@stack=\toks19
LaTeX Info: Redefining \[ on input line 2665.
LaTeX Info: Redefining \] on input line 2666.
)
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/amssymb.sty
Package: amssymb 2013/01/14 v3.01 AMS font symbols

(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/amsfonts.sty
Package: amsfonts 2013/01/14 v3.01 Basic AMSFonts support
\symAMSa=\mathgroup6
\symAMSb=\mathgroup7
LaTeX Font Info:    Overwriting math alphabet `\mathfrak' in version `bold'
(Font)                  U/euf/m/n --> U/euf/b/n on input line 106.
))
(/usr/share/texlive/texmf-dist/tex/latex/algorithms/algorithm.sty
Package: algorithm 2009/08/24 v0.1 Document Style `algorithm' - floating enviro
nment

(/usr/share/texlive/texmf-dist/tex/latex/float/float.sty
Package: float 2001/11/08 v1.3d Float enhancements (AL)
\c@float@type=\count100
\float@exts=\toks20
\float@box=\box28
\@float@everytoks=\toks21
\@floatcapt=\box29
)
(/usr/share/texlive/texmf-dist/tex/latex/base/ifthen.sty
Package: ifthen 2001/05/26 v1.1c Standard LaTeX ifthen package (DPC)
)
\@float@every@algorithm=\toks22
\c@algorithm=\count101
)
(/usr/share/texlive/texmf-dist/tex/latex/algorithms/algorithmic.sty
Package: algorithmic 2009/08/24 v0.1 Document Style `algorithmic'
\c@ALC@unique=\count102
\c@ALC@line=\count103
\c@ALC@rem=\count104
\c@ALC@depth=\count105
\ALC@tlm=\skip46
\algorithmicindent=\skip47
)
(/usr/share/texlive/texmf-dist/tex/latex/graphics/color.sty
Package: color 2005/11/14 v1.0j Standard LaTeX Color (DPC)

(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/color.cfg
File: color.cfg 2007/01/18 v1.5 color configuration of teTeX/TeXLive
)
Package color Info: Driver file: pdftex.def on input line 130.

(/usr/share/texlive/texmf-dist/tex/latex/graphics/dvipsnam.def
File: dvipsnam.def 1999/02/16 v3.0i Driver-dependant file (DPC,SPQR)
))
(/usr/share/texlive/texmf-dist/tex/latex/fancyhdr/fancyhdr.sty
\fancy@headwidth=\skip48
\f@ncyO@elh=\skip49
\f@ncyO@erh=\skip50
\f@ncyO@olh=\skip51
\f@ncyO@orh=\skip52
\f@ncyO@elf=\skip53
\f@ncyO@erf=\skip54
\f@ncyO@olf=\skip55
\f@ncyO@orf=\skip56
)
(/usr/share/texlive/texmf-dist/tex/latex/subfig/subfig.sty
Package: subfig 2005/06/28 ver: 1.3 subfig package

(/usr/share/texlive/texmf-dist/tex/latex/caption/caption.sty
Package: caption 2013/05/02 v3.3-89 Customizing captions (AR)

(/usr/share/texlive/texmf-dist/tex/latex/caption/caption3.sty
Package: caption3 2013/05/02 v1.6-88 caption3 kernel (AR)
Package caption3 Info: TeX engine: e-TeX on input line 57.
\captionmargin=\dimen114
\captionmargin@=\dimen115
\captionwidth=\dimen116
\caption@tempdima=\dimen117
\caption@indent=\dimen118
\caption@parindent=\dimen119
\caption@hangindent=\dimen120
)
\c@ContinuedFloat=\count106
Package caption Info: float package is loaded.
)
\c@KVtest=\count107
\sf@farskip=\skip57
\sf@captopadj=\dimen121
\sf@capskip=\skip58
\sf@nearskip=\skip59
\c@subfigure=\count108
\c@subfigure@save=\count109
\c@lofdepth=\count110
\c@subtable=\count111
\c@subtable@save=\count112
\c@lotdepth=\count113
\sf@top=\skip60
\sf@bottom=\skip61
)
(/usr/share/texlive/texmf-dist/tex/latex/tools/multicol.sty
Package: multicol 2011/06/27 v1.7a multicolumn formatting (FMi)
\c@tracingmulticols=\count114
\mult@box=\box30
\multicol@leftmargin=\dimen122
\c@unbalance=\count115
\c@collectmore=\count116
\doublecol@number=\count117
\multicoltolerance=\count118
\multicolpretolerance=\count119
\full@width=\dimen123
\page@free=\dimen124
\premulticols=\dimen125
\postmulticols=\dimen126
\multicolsep=\skip62
\multicolbaselineskip=\skip63
\partial@page=\box31
\last@line=\box32
\mult@rightbox=\box33
\mult@grightbox=\box34
\mult@gfirstbox=\box35
\mult@firstbox=\box36
\@tempa=\box37
\@tempa=\box38
\@tempa=\box39
\@tempa=\box40
\@tempa=\box41
\@tempa=\box42
\@tempa=\box43
\@tempa=\box44
\@tempa=\box45
\@tempa=\box46
\@tempa=\box47
\@tempa=\box48
\@tempa=\box49
\@tempa=\box50
\@tempa=\box51
\@tempa=\box52
\@tempa=\box53
\c@columnbadness=\count120
\c@finalcolumnbadness=\count121
\last@try=\dimen127
\multicolovershoot=\dimen128
\multicolundershoot=\dimen129
\mult@nat@firstbox=\box54
\colbreak@box=\box55
\multicol@sort@counter=\count122
)
(/usr/share/texlive/texmf-dist/tex/latex/multirow/multirow.sty
\bigstrutjot=\dimen130
)
(/usr/share/texlive/texmf-dist/tex/latex/wrapfig/wrapfig.sty
\wrapoverhang=\dimen131
\WF@size=\dimen132
\c@WF@wrappedlines=\count123
\WF@box=\box56
\WF@everypar=\toks23
Package: wrapfig 2003/01/31  v 3.6
)
(/usr/share/texlive/texmf-dist/tex/latex/booktabs/booktabs.sty
Package: booktabs 2005/04/14 v1.61803 publication quality tables
\heavyrulewidth=\dimen133
\lightrulewidth=\dimen134
\cmidrulewidth=\dimen135
\belowrulesep=\dimen136
\belowbottomsep=\dimen137
\aboverulesep=\dimen138
\abovetopsep=\dimen139
\cmidrulesep=\dimen140
\cmidrulekern=\dimen141
\defaultaddspace=\dimen142
\@cmidla=\count124
\@cmidlb=\count125
\@aboverulesep=\dimen143
\@belowrulesep=\dimen144
\@thisruleclass=\count126
\@lastruleclass=\count127
\@thisrulewidth=\dimen145
) (./macros.tex
(/usr/share/texlive/texmf-dist/tex/latex/tools/xspace.sty
Package: xspace 2009/10/20 v1.13 Space after command names (DPC,MH)
))
(/usr/share/texlive/texmf-dist/tex/latex/geometry/geometry.sty
Package: geometry 2010/09/12 v5.6 Page Geometry

(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/ifpdf.sty
Package: ifpdf 2011/01/30 v2.3 Provides the ifpdf switch (HO)
Package ifpdf Info: pdfTeX in PDF mode is detected.
)
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/ifvtex.sty
Package: ifvtex 2010/03/01 v1.5 Detect VTeX and its facilities (HO)
Package ifvtex Info: VTeX not detected.
)
(/usr/share/texlive/texmf-dist/tex/generic/ifxetex/ifxetex.sty
Package: ifxetex 2010/09/12 v0.6 Provides ifxetex conditional
)
\Gm@cnth=\count128
\Gm@cntv=\count129
\c@Gm@tempcnt=\count130
\Gm@bindingoffset=\dimen146
\Gm@wd@mp=\dimen147
\Gm@odd@mp=\dimen148
\Gm@even@mp=\dimen149
\Gm@layoutwidth=\dimen150
\Gm@layoutheight=\dimen151
\Gm@layouthoffset=\dimen152
\Gm@layoutvoffset=\dimen153
\Gm@dimlist=\toks24
)
(/usr/share/texlive/texmf-dist/tex/generic/ulem/ulem.sty
\UL@box=\box57
\UL@hyphenbox=\box58
\UL@skip=\skip64
\UL@hook=\toks25
\UL@height=\dimen154
\UL@pe=\count131
\UL@pixel=\dimen155
\ULC@box=\box59
Package: ulem 2012/05/18
\ULdepth=\dimen156
) (./mystyle.tex
(/usr/share/texlive/texmf-dist/tex/latex/dblfloatfix/dblfloatfix.sty
Package: dblfloatfix 2012/12/31 v1.0a (JAW)

(/usr/share/texlive/texmf-dist/tex/latex/base/fixltx2e.sty
Package: fixltx2e 2006/09/13 v1.1m fixes to LaTeX
LaTeX Info: Redefining \em on input line 420.
)
\@dblbotnum=\count132
\c@dblbotnumber=\count133
)
(/usr/share/texlive/texmf-dist/tex/latex/setspace/setspace.sty
Package: setspace 2011/12/19 v6.7a set line spacing
)
(/usr/share/texlive/texmf-dist/tex/latex/psnfss/pifont.sty
Package: pifont 2005/04/12 PSNFSS-v9.2a Pi font support (SPQR) 
LaTeX Font Info:    Try loading font information for U+pzd on input line 63.

(/usr/share/texlive/texmf-dist/tex/latex/psnfss/upzd.fd
File: upzd.fd 2001/06/04 font definitions for U/pzd.
)
LaTeX Font Info:    Try loading font information for U+psy on input line 64.

(/usr/share/texlive/texmf-dist/tex/latex/psnfss/upsy.fd
File: upsy.fd 2001/06/04 font definitions for U/psy.
))
(/usr/share/texlive/texmf-dist/tex/latex/l3packages/xfrac/xfrac.sty
(/usr/share/texlive/texmf-dist/tex/latex/l3packages/l3keys2e/l3keys2e.sty
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/expl3.sty
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3names.sty
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3bootstrap.sty
Package: l3bootstrap 2014/01/04 v4640 L3 Experimental bootstrap code
)
Package: l3names 2014/01/04 v4640 L3 Namespace for primitives
)
(/usr/share/texlive/texmf-dist/tex/latex/etex-pkg/etex.sty
Package: etex 1998/03/26 v2.0 eTeX basic definition package (PEB)
\et@xins=\count134
)
Package: expl3 2014/01/07 v4646 L3 Experimental code bundle wrapper

(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3basics.sty
Package: l3basics 2014/01/04 v4642 L3 Basic definitions
)
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3expan.sty
Package: l3expan 2014/01/04 v4642 L3 Argument expansion
)
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3tl.sty
Package: l3tl 2013/12/27 v4625 L3 Token lists
)
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3seq.sty
Package: l3seq 2013/12/14 v4623 L3 Sequences and stacks
)
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3int.sty
Package: l3int 2013/08/02 v4583 L3 Integers
\c_max_int=\count135
\l_tmpa_int=\count136
\l_tmpb_int=\count137
\g_tmpa_int=\count138
\g_tmpb_int=\count139
)
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3quark.sty
Package: l3quark 2013/12/14 v4623 L3 Quarks
)
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3prg.sty
Package: l3prg 2014/01/04 v4642 L3 Control structures
\g__prg_map_int=\count140
)
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3clist.sty
Package: l3clist 2013/07/28 v4581 L3 Comma separated lists
)
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3token.sty
Package: l3token 2013/08/25 v4587 L3 Experimental token manipulation
)
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3prop.sty
Package: l3prop 2013/12/14 v4623 L3 Property lists
)
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3msg.sty
Package: l3msg 2013/07/28 v4581 L3 Messages
)
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3file.sty
Package: l3file 2013/10/13 v4596 L3 File and I/O operations
\l_iow_line_count_int=\count141
\l__iow_target_count_int=\count142
\l__iow_current_line_int=\count143
\l__iow_current_word_int=\count144
\l__iow_current_indentation_int=\count145
)
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3skip.sty
Package: l3skip 2013/07/28 v4581 L3 Dimensions and skips
\c_zero_dim=\dimen157
\c_max_dim=\dimen158
\l_tmpa_dim=\dimen159
\l_tmpb_dim=\dimen160
\g_tmpa_dim=\dimen161
\g_tmpb_dim=\dimen162
\c_zero_skip=\skip65
\c_max_skip=\skip66
\l_tmpa_skip=\skip67
\l_tmpb_skip=\skip68
\g_tmpa_skip=\skip69
\g_tmpb_skip=\skip70
\c_zero_muskip=\muskip12
\c_max_muskip=\muskip13
\l_tmpa_muskip=\muskip14
\l_tmpb_muskip=\muskip15
\g_tmpa_muskip=\muskip16
\g_tmpb_muskip=\muskip17
)
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3keys.sty
Package: l3keys 2013/12/08 v4614 L3 Experimental key-value interfaces
\g__keyval_level_int=\count146
\l_keys_choice_int=\count147
)
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3fp.sty
Package: l3fp 2014/01/04 v4642 L3 Floating points
\c__fp_leading_shift_int=\count148
\c__fp_middle_shift_int=\count149
\c__fp_trailing_shift_int=\count150
\c__fp_big_leading_shift_int=\count151
\c__fp_big_middle_shift_int=\count152
\c__fp_big_trailing_shift_int=\count153
\c__fp_Bigg_leading_shift_int=\count154
\c__fp_Bigg_middle_shift_int=\count155
\c__fp_Bigg_trailing_shift_int=\count156
)
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3box.sty
Package: l3box 2013/07/28 v4581 L3 Experimental boxes
\c_empty_box=\box60
\l_tmpa_box=\box61
\l_tmpb_box=\box62
\g_tmpa_box=\box63
\g_tmpb_box=\box64
)
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3coffins.sty
Package: l3coffins 2013/12/14 v4624 L3 Coffin code layer
\l__coffin_internal_box=\box65
\l__coffin_internal_dim=\dimen163
\l__coffin_offset_x_dim=\dimen164
\l__coffin_offset_y_dim=\dimen165
\l__coffin_x_dim=\dimen166
\l__coffin_y_dim=\dimen167
\l__coffin_x_prime_dim=\dimen168
\l__coffin_y_prime_dim=\dimen169
\c_empty_coffin=\box66
\l__coffin_aligned_coffin=\box67
\l__coffin_aligned_internal_coffin=\box68
\l_tmpa_coffin=\box69
\l_tmpb_coffin=\box70
\l__coffin_display_coffin=\box71
\l__coffin_display_coord_coffin=\box72
\l__coffin_display_pole_coffin=\box73
\l__coffin_display_offset_dim=\dimen170
\l__coffin_display_x_dim=\dimen171
\l__coffin_display_y_dim=\dimen172
)
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3color.sty
Package: l3color 2012/08/29 v4156 L3 Experimental color support
)
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3luatex.sty
Package: l3luatex 2013/07/28 v4581 L3 Experimental LuaTeX-specific functions
\g__cctab_allocate_int=\count157
\g__cctab_stack_int=\count158
)
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3candidates.sty
Package: l3candidates 2014/01/06 v4643 L3 Experimental additions to l3kernel
\l__box_top_dim=\dimen173
\l__box_bottom_dim=\dimen174
\l__box_left_dim=\dimen175
\l__box_right_dim=\dimen176
\l__box_top_new_dim=\dimen177
\l__box_bottom_new_dim=\dimen178
\l__box_left_new_dim=\dimen179
\l__box_right_new_dim=\dimen180
\l__box_internal_box=\box74
\l__coffin_bounding_shift_dim=\dimen181
\l__coffin_left_corner_dim=\dimen182
\l__coffin_right_corner_dim=\dimen183
\l__coffin_bottom_corner_dim=\dimen184
\l__coffin_top_corner_dim=\dimen185
\l__coffin_scaled_total_height_dim=\dimen186
\l__coffin_scaled_width_dim=\dimen187
))
Package: l3keys2e 2013/12/31 v4634 LaTeX2e option processing using LaTeX3 keys
)
(/usr/share/texlive/texmf-dist/tex/latex/base/textcomp.sty
Package: textcomp 2005/09/27 v1.99g Standard LaTeX package
Package textcomp Info: Sub-encoding information:
(textcomp)               5 = only ISO-Adobe without \textcurrency
(textcomp)               4 = 5 + \texteuro
(textcomp)               3 = 4 + \textohm
(textcomp)               2 = 3 + \textestimated + \textcurrency
(textcomp)               1 = TS1 - \textcircled - \t
(textcomp)               0 = TS1 (full)
(textcomp)             Font families with sub-encoding setting implement
(textcomp)             only a restricted character set as indicated.
(textcomp)             Family '?' is the default used for unknown fonts.
(textcomp)             See the documentation for details.
Package textcomp Info: Setting ? sub-encoding to TS1/1 on input line 71.

(/usr/share/texlive/texmf-dist/tex/latex/base/ts1enc.def
File: ts1enc.def 2001/06/05 v3.0e (jk/car/fm) Standard LaTeX file
)
LaTeX Info: Redefining \oldstylenums on input line 266.
Package textcomp Info: Setting cmr sub-encoding to TS1/0 on input line 281.
Package textcomp Info: Setting cmss sub-encoding to TS1/0 on input line 282.
Package textcomp Info: Setting cmtt sub-encoding to TS1/0 on input line 283.
Package textcomp Info: Setting cmvtt sub-encoding to TS1/0 on input line 284.
Package textcomp Info: Setting cmbr sub-encoding to TS1/0 on input line 285.
Package textcomp Info: Setting cmtl sub-encoding to TS1/0 on input line 286.
Package textcomp Info: Setting ccr sub-encoding to TS1/0 on input line 287.
Package textcomp Info: Setting ptm sub-encoding to TS1/4 on input line 288.
Package textcomp Info: Setting pcr sub-encoding to TS1/4 on input line 289.
Package textcomp Info: Setting phv sub-encoding to TS1/4 on input line 290.
Package textcomp Info: Setting ppl sub-encoding to TS1/3 on input line 291.
Package textcomp Info: Setting pag sub-encoding to TS1/4 on input line 292.
Package textcomp Info: Setting pbk sub-encoding to TS1/4 on input line 293.
Package textcomp Info: Setting pnc sub-encoding to TS1/4 on input line 294.
Package textcomp Info: Setting pzc sub-encoding to TS1/4 on input line 295.
Package textcomp Info: Setting bch sub-encoding to TS1/4 on input line 296.
Package textcomp Info: Setting put sub-encoding to TS1/5 on input line 297.
Package textcomp Info: Setting uag sub-encoding to TS1/5 on input line 298.
Package textcomp Info: Setting ugq sub-encoding to TS1/5 on input line 299.
Package textcomp Info: Setting ul8 sub-encoding to TS1/4 on input line 300.
Package textcomp Info: Setting ul9 sub-encoding to TS1/4 on input line 301.
Package textcomp Info: Setting augie sub-encoding to TS1/5 on input line 302.
Package textcomp Info: Setting dayrom sub-encoding to TS1/3 on input line 303.
Package textcomp Info: Setting dayroms sub-encoding to TS1/3 on input line 304.

Package textcomp Info: Setting pxr sub-encoding to TS1/0 on input line 305.
Package textcomp Info: Setting pxss sub-encoding to TS1/0 on input line 306.
Package textcomp Info: Setting pxtt sub-encoding to TS1/0 on input line 307.
Package textcomp Info: Setting txr sub-encoding to TS1/0 on input line 308.
Package textcomp Info: Setting txss sub-encoding to TS1/0 on input line 309.
Package textcomp Info: Setting txtt sub-encoding to TS1/0 on input line 310.
Package textcomp Info: Setting lmr sub-encoding to TS1/0 on input line 311.
Package textcomp Info: Setting lmdh sub-encoding to TS1/0 on input line 312.
Package textcomp Info: Setting lmss sub-encoding to TS1/0 on input line 313.
Package textcomp Info: Setting lmssq sub-encoding to TS1/0 on input line 314.
Package textcomp Info: Setting lmvtt sub-encoding to TS1/0 on input line 315.
Package textcomp Info: Setting qhv sub-encoding to TS1/0 on input line 316.
Package textcomp Info: Setting qag sub-encoding to TS1/0 on input line 317.
Package textcomp Info: Setting qbk sub-encoding to TS1/0 on input line 318.
Package textcomp Info: Setting qcr sub-encoding to TS1/0 on input line 319.
Package textcomp Info: Setting qcs sub-encoding to TS1/0 on input line 320.
Package textcomp Info: Setting qpl sub-encoding to TS1/0 on input line 321.
Package textcomp Info: Setting qtm sub-encoding to TS1/0 on input line 322.
Package textcomp Info: Setting qzc sub-encoding to TS1/0 on input line 323.
Package textcomp Info: Setting qhvc sub-encoding to TS1/0 on input line 324.
Package textcomp Info: Setting futs sub-encoding to TS1/4 on input line 325.
Package textcomp Info: Setting futx sub-encoding to TS1/4 on input line 326.
Package textcomp Info: Setting futj sub-encoding to TS1/4 on input line 327.
Package textcomp Info: Setting hlh sub-encoding to TS1/3 on input line 328.
Package textcomp Info: Setting hls sub-encoding to TS1/3 on input line 329.
Package textcomp Info: Setting hlst sub-encoding to TS1/3 on input line 330.
Package textcomp Info: Setting hlct sub-encoding to TS1/5 on input line 331.
Package textcomp Info: Setting hlx sub-encoding to TS1/5 on input line 332.
Package textcomp Info: Setting hlce sub-encoding to TS1/5 on input line 333.
Package textcomp Info: Setting hlcn sub-encoding to TS1/5 on input line 334.
Package textcomp Info: Setting hlcw sub-encoding to TS1/5 on input line 335.
Package textcomp Info: Setting hlcf sub-encoding to TS1/5 on input line 336.
Package textcomp Info: Setting pplx sub-encoding to TS1/3 on input line 337.
Package textcomp Info: Setting pplj sub-encoding to TS1/3 on input line 338.
Package textcomp Info: Setting ptmx sub-encoding to TS1/4 on input line 339.
Package textcomp Info: Setting ptmj sub-encoding to TS1/4 on input line 340.
)
(/usr/share/texlive/texmf-dist/tex/latex/l3packages/xparse/xparse.sty
Package: xparse 2013/12/31 v4634 L3 Experimental document command parser
\l__xparse_current_arg_int=\count159
\l__xparse_m_args_int=\count160
\l__xparse_mandatory_args_int=\count161
\l__xparse_processor_int=\count162
\l__xparse_v_nesting_int=\count163
)
(/usr/share/texlive/texmf-dist/tex/latex/l3packages/xtemplate/xtemplate.sty
Package: xtemplate 2013/12/31 v4634 L3 Experimental prototype document function
s
\l__xtemplate_tmp_dim=\dimen188
\l__xtemplate_tmp_int=\count164
\l__xtemplate_tmp_muskip=\muskip18
\l__xtemplate_tmp_skip=\skip71
Variant \prop_get:NoNTF already defined; not changing it on line 106
Variant \prop_get:NoNT already defined; not changing it on line 107
Variant \prop_get:NoNF already defined; not changing it on line 108
)
Package: xfrac 2012/11/09 v4299 L3 Experimental split-level fractions
\l__xfrac_slash_box=\box75
\l__xfrac_tmp_box=\box76
\l__xfrac_denominator_bot_sep_dim=\dimen189
\l__xfrac_numerator_bot_sep_dim=\dimen190
\l__xfrac_numerator_top_sep_dim=\dimen191
\l__xfrac_slash_left_sep_dim=\dimen192
\l__xfrac_slash_right_sep_dim=\dimen193
\l__xfrac_slash_left_muskip=\muskip19
\l__xfrac_slash_right_muskip=\muskip20
.................................................
. xtemplate info: "declare-object-type"
. 
. Declaring object type 'xfrac' taking 3 argument(s) on line 96.
.................................................
.................................................
. LaTeX info: "xparse/define-command"
. 
. Defining document command \sfrac with arg. spec. 'omom' on line 436.
.................................................
))
(./paper.aux)
\openout1 = `paper.aux'.

LaTeX Font Info:    Checking defaults for OML/cmm/m/it on input line 40.
LaTeX Font Info:    ... okay on input line 40.
LaTeX Font Info:    Checking defaults for T1/cmr/m/n on input line 40.
LaTeX Font Info:    ... okay on input line 40.
LaTeX Font Info:    Checking defaults for OT1/cmr/m/n on input line 40.
LaTeX Font Info:    ... okay on input line 40.
LaTeX Font Info:    Checking defaults for OMS/pzccm/m/n on input line 40.
LaTeX Font Info:    Try loading font information for OMS+pzccm on input line 40
.
 (/usr/share/texlive/texmf-dist/tex/latex/psnfss/omspzccm.fd
File: omspzccm.fd 2000/01/03 Fontinst v1.801 font definitions for OMS/pzccm.
)
LaTeX Font Info:    ... okay on input line 40.
LaTeX Font Info:    Checking defaults for OMX/cmex/m/n on input line 40.
LaTeX Font Info:    ... okay on input line 40.
LaTeX Font Info:    Checking defaults for U/cmr/m/n on input line 40.
LaTeX Font Info:    ... okay on input line 40.
LaTeX Font Info:    Checking defaults for TS1/cmr/m/n on input line 40.
LaTeX Font Info:    Try loading font information for TS1+cmr on input line 40.

(/usr/share/texlive/texmf-dist/tex/latex/base/ts1cmr.fd
File: ts1cmr.fd 1999/05/25 v2.5h Standard LaTeX font definitions
)
LaTeX Font Info:    ... okay on input line 40.

(/usr/share/texlive/texmf-dist/tex/context/base/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
\scratchcounter=\count165
\scratchdimen=\dimen194
\scratchbox=\box77
\nofMPsegments=\count166
\nofMParguments=\count167
\everyMPshowfont=\toks26
\MPscratchCnt=\count168
\MPscratchDim=\dimen195
\MPnumerator=\count169
\makeMPintoPDFobject=\count170
\everyMPtoPDFconversion=\toks27
) (/usr/share/texlive/texmf-dist/tex/generic/oberdiek/pdftexcmds.sty
Package: pdftexcmds 2011/11/29 v0.20 Utility functions of pdfTeX for LuaTeX (HO
)

(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/ifluatex.sty
Package: ifluatex 2010/03/01 v1.3 Provides the ifluatex switch (HO)
Package ifluatex Info: LuaTeX not detected.
)
Package pdftexcmds Info: LuaTeX not detected.
Package pdftexcmds Info: \pdf@primitive is available.
Package pdftexcmds Info: \pdf@ifprimitive is available.
Package pdftexcmds Info: \pdfdraftmode found.
)
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/epstopdf-base.sty
Package: epstopdf-base 2010/02/09 v2.5 Base part for package epstopdf

(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/grfext.sty
Package: grfext 2010/08/19 v1.1 Manage graphics extensions (HO)

(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/kvdefinekeys.sty
Package: kvdefinekeys 2011/04/07 v1.3 Define keys (HO)
))
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/kvoptions.sty
Package: kvoptions 2011/06/30 v3.11 Key value format for package options (HO)

(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/kvsetkeys.sty
Package: kvsetkeys 2012/04/25 v1.16 Key value parser (HO)

(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/etexcmds.sty
Package: etexcmds 2011/02/16 v1.5 Avoid name clashes with e-TeX commands (HO)
Package etexcmds Info: Could not find \expanded.
(etexcmds)             That can mean that you are not using pdfTeX 1.50 or
(etexcmds)             that some package has redefined \expanded.
(etexcmds)             In the latter case, load this package earlier.
)))
Package grfext Info: Graphics extension search list:
(grfext)             [.png,.pdf,.jpg,.mps,.jpeg,.jbig2,.jb2,.PNG,.PDF,.JPG,.JPE
G,.JBIG2,.JB2,.eps]
(grfext)             \AppendGraphicsExtensions on input line 452.

(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg
File: epstopdf-sys.cfg 2010/07/13 v1.3 Configuration of (r)epstopdf for TeX Liv
e
))
Package caption Info: Begin \AtBeginDocument code.
Package caption Info: subfig package v1.3 is loaded.
Package caption Info: wrapfig package is loaded.
Package caption Info: End \AtBeginDocument code.

*geometry* driver: auto-detecting
*geometry* detected driver: pdftex
*geometry* verbose mode - [ preamble ] result:
* driver: pdftex
* paper: letterpaper
* layout: <same size as paper>
* layoutoffset:(h,v)=(0.0pt,0.0pt)
* modes: 
* h-part:(L,W,R)=(72.26999pt, 469.75502pt, 72.26999pt)
* v-part:(T,H,B)=(72.26999pt, 650.43001pt, 72.26999pt)
* \paperwidth=614.295pt
* \paperheight=794.96999pt
* \textwidth=469.75502pt
* \textheight=650.43001pt
* \oddsidemargin=0.0pt
* \evensidemargin=0.0pt
* \topmargin=-37.0pt
* \headheight=12.0pt
* \headsep=25.0pt
* \topskip=10.0pt
* \footskip=30.0pt
* \marginparwidth=65.0pt
* \marginparsep=11.0pt
* \columnsep=10.0pt
* \skip\footins=9.0pt plus 4.0pt minus 2.0pt
* \hoffset=0.0pt
* \voffset=0.0pt
* \mag=1000
* \@twocolumnfalse
* \@twosidefalse
* \@mparswitchfalse
* \@reversemarginfalse
* (1in=72.27pt=25.4mm, 1cm=28.453pt)

LaTeX Font Info:    Try loading font information for OT1+ptmcm on input line 64
.
(/usr/share/texlive/texmf-dist/tex/latex/psnfss/ot1ptmcm.fd
File: ot1ptmcm.fd 2000/01/03 Fontinst v1.801 font definitions for OT1/ptmcm.
)
LaTeX Font Info:    Try loading font information for OML+ptmcm on input line 64
.

(/usr/share/texlive/texmf-dist/tex/latex/psnfss/omlptmcm.fd
File: omlptmcm.fd 2000/01/03 Fontinst v1.801 font definitions for OML/ptmcm.
)
LaTeX Font Info:    Try loading font information for OMX+psycm on input line 64
.

(/usr/share/texlive/texmf-dist/tex/latex/psnfss/omxpsycm.fd
File: omxpsycm.fd 2000/01/03 Fontinst v1.801 font definitions for OMX/psycm.
)
LaTeX Font Info:    Font shape `OT1/ptm/bx/n' in size <12> not available
(Font)              Font shape `OT1/ptm/b/n' tried instead on input line 64.
LaTeX Font Info:    Font shape `OT1/ptm/bx/n' in size <9> not available
(Font)              Font shape `OT1/ptm/b/n' tried instead on input line 64.
LaTeX Font Info:    Font shape `OT1/ptm/bx/n' in size <7> not available
(Font)              Font shape `OT1/ptm/b/n' tried instead on input line 64.
LaTeX Font Info:    Try loading font information for U+msa on input line 64.

(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/umsa.fd
File: umsa.fd 2013/01/14 v3.01 AMS symbols A
)
LaTeX Font Info:    Try loading font information for U+msb on input line 64.

(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/umsb.fd
File: umsb.fd 2013/01/14 v3.01 AMS symbols B
) (./0_abstract.tex)
(./1_intro.tex
LaTeX Font Info:    Font shape `OT1/ptm/bx/n' in size <14.4> not available
(Font)              Font shape `OT1/ptm/b/n' tried instead on input line 1.
LaTeX Font Info:    Font shape `OT1/ptm/bx/n' in size <10> not available
(Font)              Font shape `OT1/ptm/b/n' tried instead on input line 10.
LaTeX Font Info:    Font shape `OT1/ptm/bx/n' in size <7.4> not available
(Font)              Font shape `OT1/ptm/b/n' tried instead on input line 10.
LaTeX Font Info:    Font shape `OT1/ptm/bx/n' in size <6> not available
(Font)              Font shape `OT1/ptm/b/n' tried instead on input line 10.
LaTeX Font Info:    Font shape `OT1/ptm/bx/n' in size <8> not available
(Font)              Font shape `OT1/ptm/b/n' tried instead on input line 41.
LaTeX Font Info:    Font shape `OT1/ptm/bx/n' in size <5> not available
(Font)              Font shape `OT1/ptm/b/n' tried instead on input line 41.
 [1{/var/lib/texmf/fonts/map/pdftex/updmap/pdftex.map}

]
(./summary.tex <baseline.pdf, id=11, 145.54375pt x 150.5625pt>
File: baseline.pdf Graphic file (type pdf)

<use baseline.pdf>
Package pdftex.def Info: baseline.pdf used on input line 7.
(pdftex.def)             Requested size: 125.76257pt x 130.08621pt.
 <dedicated.pdf, id=12, 103.38625pt x 150.5625pt>
File: dedicated.pdf Graphic file (type pdf)

<use dedicated.pdf>
Package pdftex.def Info: dedicated.pdf used on input line 11.
(pdftex.def)             Requested size: 89.3348pt x 130.08621pt.
 <cascaded.pdf, id=13, 104.39pt x 150.5625pt>
File: cascaded.pdf Graphic file (type pdf)

<use cascaded.pdf>
Package pdftex.def Info: cascaded.pdf used on input line 15.
(pdftex.def)             Requested size: 90.2021pt x 130.08621pt.
) [2 <./baseline.pdf> <./dedicated.pdf> <./cascaded.pdf>])
(./2_background.tex (./stack.tex
<stack_four.pdf, id=35, 189.70876pt x 111.41624pt>
File: stack_four.pdf Graphic file (type pdf)
 <use stack_four.pdf>
Package pdftex.def Info: stack_four.pdf used on input line 7.
(pdftex.def)             Requested size: 147.66537pt x 86.72377pt.

<stack_two.pdf, id=36, 112.42pt x 112.42pt>
File: stack_two.pdf Graphic file (type pdf)
 <use stack_two.pdf>
Package pdftex.def Info: stack_two.pdf used on input line 11.
(pdftex.def)             Requested size: 86.72662pt x 86.72377pt.
) [3 <./stack_four.pdf> <./stack_two.pdf>] (./dram.tex
<dram_io.pdf, id=52, 190.7125pt x 192.72pt>
File: dram_io.pdf Graphic file (type pdf)
 <use dram_io.pdf>
Package pdftex.def Info: dram_io.pdf used on input line 7.
(pdftex.def)             Requested size: 121.57832pt x 122.85876pt.

<dram_timing.pdf, id=53, 419.5675pt x 190.7125pt>
File: dram_timing.pdf Graphic file (type pdf)
 <use dram_timing.pdf>
Package pdftex.def Info: dram_timing.pdf used on input line 12.
(pdftex.def)             Requested size: 270.28925pt x 122.85876pt.
)
[4 <./dram_io.pdf> <./dram_timing.pdf>] (./trend_bandwidth.tex
<bandwidth.pdf, id=70, 359.3425pt x 184.69pt>
File: bandwidth.pdf Graphic file (type pdf)
 <use bandwidth.pdf>
Package pdftex.def Info: bandwidth.pdf used on input line 3.
(pdftex.def)             Requested size: 305.33789pt x 156.94495pt.
) [5 <./bandwidth.pdf>]) (./3_motivation.tex (./motivation.tex
<multirank.pdf, id=85, 117.43875pt x 103.38625pt>
File: multirank.pdf Graphic file (type pdf)
 <use multirank.pdf>
Package pdftex.def Info: multirank.pdf used on input line 8.
(pdftex.def)             Requested size: 98.51346pt x 86.72377pt.

<multirank_3d.pdf, id=86, 129.48375pt x 100.375pt>
File: multirank_3d.pdf Graphic file (type pdf)
 <use multirank_3d.pdf>
Package pdftex.def Info: multirank_3d.pdf used on input line 12.
(pdftex.def)             Requested size: 111.88136pt x 86.72377pt.

<multirank_dio.pdf, id=87, 119.44624pt x 100.375pt>
File: multirank_dio.pdf Graphic file (type pdf)
 <use multirank_dio.pdf>
Package pdftex.def Info: multirank_dio.pdf used on input line 24.
(pdftex.def)             Requested size: 103.20839pt x 86.72377pt.

<multirank_cio.pdf, id=88, 119.44624pt x 100.375pt>
File: multirank_cio.pdf Graphic file (type pdf)
 <use multirank_cio.pdf>
Package pdftex.def Info: multirank_cio.pdf used on input line 28.
(pdftex.def)             Requested size: 103.20839pt x 86.72377pt.

Overfull \hbox (1.63751pt too wide) in paragraph at lines 2--33
[]$[]$   $[]$
 []

) [6 <./multirank.pdf> <./multirank_3d.pdf> <./multirank_dio.pdf> <./multirank_
cio.pdf>]) (./4_smla.tex
LaTeX Font Info:    Calculating math sizes for size <6.99997> on input line 49.

LaTeX Font Info:    Font shape `OT1/ptm/bx/n' in size <6.99997> not available
(Font)              Font shape `OT1/ptm/b/n' tried instead on input line 49.
LaTeX Font Info:    Font shape `OT1/ptm/bx/n' in size <4.89995> not available
(Font)              Font shape `OT1/ptm/b/n' tried instead on input line 49.
LaTeX Font Info:    Font shape `OT1/ptm/bx/n' in size <3.49998> not available
(Font)              Font shape `OT1/ptm/b/n' tried instead on input line 49.
 (./dio.tex
<sio_detail.pdf, id=116, 187.70125pt x 104.39pt>
File: sio_detail.pdf Graphic file (type pdf)
 <use sio_detail.pdf>
Package pdftex.def Info: sio_detail.pdf used on input line 8.
(pdftex.def)             Requested size: 142.94943pt x 79.49744pt.

<dio_detail.pdf, id=117, 187.70125pt x 104.39pt>
File: dio_detail.pdf Graphic file (type pdf)
 <use dio_detail.pdf>
Package pdftex.def Info: dio_detail.pdf used on input line 12.
(pdftex.def)             Requested size: 142.94943pt x 79.49744pt.
) [7 <./sio_detail.pdf> <./dio_detail.pdf>] (./cio.tex
<cio_org.pdf, id=134, 133.49875pt x 129.48375pt>
File: cio_org.pdf Graphic file (type pdf)
 <use cio_org.pdf>
Package pdftex.def Info: cio_org.pdf used on input line 7.
(pdftex.def)             Requested size: 119.22293pt x 115.63243pt.

<cio_sclk.pdf, id=135, 178.6675pt x 125.46875pt>
File: cio_sclk.pdf Graphic file (type pdf)
 <use cio_sclk.pdf>
Package pdftex.def Info: cio_sclk.pdf used on input line 11.
(pdftex.def)             Requested size: 164.66779pt x 115.63243pt.

<cio_rclk.pdf, id=136, 167.62625pt x 124.465pt>
File: cio_rclk.pdf Graphic file (type pdf)
 <use cio_rclk.pdf>
Package pdftex.def Info: cio_rclk.pdf used on input line 15.
(pdftex.def)             Requested size: 155.73476pt x 115.63243pt.
) [8 <./cio_org.pdf> <./cio_sclk.pdf> <./cio_rclk.pdf>]) (./5_rank.tex [9]
(./timeline_rank.tex <dio_mlr.pdf, id=173, 219.82124pt x 28.105pt>
File: dio_mlr.pdf Graphic file (type pdf)

<use dio_mlr.pdf>
Package pdftex.def Info: dio_mlr.pdf used on input line 7.
(pdftex.def)             Requested size: 258.36668pt x 33.03407pt.
 <dio_slr.pdf, id=174, 215.80624pt x 23.08624pt>
File: dio_slr.pdf Graphic file (type pdf)

<use dio_slr.pdf>
Package pdftex.def Info: dio_slr.pdf used on input line 13.
(pdftex.def)             Requested size: 258.36668pt x 27.64203pt.
 <cio_slr.pdf, id=175, 219.82124pt x 30.1125pt>
File: cio_slr.pdf Graphic file (type pdf)

<use cio_slr.pdf>
Package pdftex.def Info: cio_slr.pdf used on input line 19.
(pdftex.def)             Requested size: 258.36668pt x 35.39366pt.
 <timeline_legend.pdf, id=176, 216.81pt x 10.0375pt>
File: timeline_legend.pdf Graphic file (type pdf)

<use timeline_legend.pdf>
Package pdftex.def Info: timeline_legend.pdf used on input line 24.
(pdftex.def)             Requested size: 258.36668pt x 11.96281pt.
) [10 <./dio_mlr.pdf> <./dio_slr.pdf> <./cio_slr.pdf> <./timeline_legend.pdf>])
 (./6_energy.tex (./trend_current.tex
<trend_current.pdf, id=221, 599.23875pt x 200.75pt>
File: trend_current.pdf Graphic file (type pdf)
 <use trend_current.pdf>
Package pdftex.def Info: trend_current.pdf used on input line 3.
(pdftex.def)             Requested size: 305.33789pt x 102.2923pt.
)
(./energy.tex)) (./7_method.tex [11 <./trend_current.pdf>] (./memory.tex)
(./system.tex)) (./8_result.tex [12] (./result_single.tex
<result_perf_mlr.pdf, id=238, 616.3025pt x 216.81pt>
File: result_perf_mlr.pdf Graphic file (type pdf)
 <use result_perf_mlr.pdf>
Package pdftex.def Info: result_perf_mlr.pdf used on input line 10.
(pdftex.def)             Requested size: 211.38832pt x 74.36284pt.

<result_energy_mlr.pdf, id=239, 611.28375pt x 336.25626pt>
File: result_energy_mlr.pdf Graphic file (type pdf)

<use result_energy_mlr.pdf>
Package pdftex.def Info: result_energy_mlr.pdf used on input line 10.
(pdftex.def)             Requested size: 211.38832pt x 116.28046pt.

<result_perf_slr.pdf, id=240, 616.3025pt x 216.81pt>
File: result_perf_slr.pdf Graphic file (type pdf)
 <use result_perf_slr.pdf>
Package pdftex.def Info: result_perf_slr.pdf used on input line 17.
(pdftex.def)             Requested size: 211.38832pt x 74.36284pt.

<result_energy_slr.pdf, id=241, 611.28375pt x 336.25626pt>
File: result_energy_slr.pdf Graphic file (type pdf)

<use result_energy_slr.pdf>
Package pdftex.def Info: result_energy_slr.pdf used on input line 17.
(pdftex.def)             Requested size: 211.38832pt x 116.28046pt.
) [13 <./result_perf_mlr.pdf> <./result_energy_mlr.pdf> <./result_perf_slr.pdf>
 <./result_energy_slr.pdf>] (./result_multi.tex
<result_ipc_multi.pdf, id=258, 360.34625pt x 268.00125pt>
File: result_ipc_multi.pdf Graphic file (type pdf)

<use result_ipc_multi.pdf>
Package pdftex.def Info: result_ipc_multi.pdf used on input line 8.
(pdftex.def)             Requested size: 140.92793pt x 104.8104pt.

<result_pwr_multi.pdf, id=259, 360.34625pt x 268.00125pt>
File: result_pwr_multi.pdf Graphic file (type pdf)

<use result_pwr_multi.pdf>
Package pdftex.def Info: result_pwr_multi.pdf used on input line 12.
(pdftex.def)             Requested size: 140.92793pt x 104.8104pt.
) (./result_layer.tex
<result_ipc_layer.pdf, id=260, 360.34625pt x 268.00125pt>
File: result_ipc_layer.pdf Graphic file (type pdf)

<use result_ipc_layer.pdf>
Package pdftex.def Info: result_ipc_layer.pdf used on input line 8.
(pdftex.def)             Requested size: 140.92793pt x 104.8104pt.

<result_pwr_layer.pdf, id=261, 360.34625pt x 268.00125pt>
File: result_pwr_layer.pdf Graphic file (type pdf)

<use result_pwr_layer.pdf>
Package pdftex.def Info: result_pwr_layer.pdf used on input line 12.
(pdftex.def)             Requested size: 140.92793pt x 104.8104pt.
) [14 <./result_ipc_multi.pdf> <./result_pwr_multi.pdf>] (./result_energy.tex <
result_energy.pdf, id=271, 656.4525pt x 156.585pt>
File: result_energy.pdf Graphic file (type pdf)

<use result_energy.pdf>
Package pdftex.def Info: result_energy.pdf used on input line 7.
(pdftex.def)             Requested size: 281.85587pt x 67.23227pt.

<result_energy_increase.pdf, id=272, 617.30624pt x 145.54375pt>
File: result_energy_increase.pdf Graphic file (type pdf)

<use result_energy_increase.pdf>
Package pdftex.def Info: result_energy_increase.pdf used on input line 13.
(pdftex.def)             Requested size: 281.85587pt x 66.45569pt.
)) (./9_related.tex [15 <./result_ipc_layer.pdf> <./result_pwr_layer.pdf> <./re
sult_energy.pdf> <./result_energy_increase.pdf>]) (./10_conclusion.tex) (./11_a
ck.tex) [16] (./paper.bbl [17]) [18]
(./paper.aux) ) 
Here is how much of TeX's memory you used:
 12199 strings out of 493304
 219350 string characters out of 6139871
 268800 words of memory out of 5000000
 15260 multiletter control sequences out of 15000+600000
 96041 words of font info for 217 fonts, out of 8000000 for 9000
 957 hyphenation exceptions out of 8191
 47i,13n,47p,10453b,459s stack positions out of 5000i,500n,10000p,200000b,80000s
{/usr/share/texlive/texmf-dist/fonts/enc/dvips/base/8r.enc}</usr
/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi10.pfb></usr/share
/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmr10.pfb></usr/share/texliv
e/texmf-dist/fonts/type1/public/amsfonts/cm/cmsy10.pfb></usr/share/texlive/texm
f-dist/fonts/type1/urw/courier/ucrr8a.pfb></usr/share/texlive/texmf-dist/fonts/
type1/urw/times/utmb8a.pfb></usr/share/texlive/texmf-dist/fonts/type1/urw/times
/utmr8a.pfb></usr/share/texlive/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on paper.pdf (18 pages, 1515943 bytes).
PDF statistics:
 328 PDF objects out of 1000 (max. 8388607)
 193 compressed objects within 2 object streams
 0 named destinations out of 1000 (max. 500000)
 161 words of extra memory for PDF output out of 10000 (max. 10000000)


